Are all outliers alike? On Understanding the Diversity of Outliers for Detecting OODs

Deep neural networks (DNNs) are known to produce incorrect predictions with very high confidence on out-of-distribution (OOD) inputs. This limitation is one of the key challenges in the adoption of deep learning models in high-assurance systems such as autonomous driving, air traffic management, and medical diagnosis. This challenge has received significant attention recently, and several techniques have been developed to detect inputs where the model's prediction cannot be trusted. These techniques use different statistical, geometric, or topological signatures. This paper presents a taxonomy of OOD outlier inputs based on their source and nature of uncertainty. We demonstrate how different existing detection approaches fail to detect certain types of outliers. We utilize these insights to develop a novel integrated detection approach that uses multiple attributes corresponding to different types of outliers. Our results include experiments on CIFAR10, SVHN and MNIST as in-distribution data and Imagenet, LSUN, SVHN (for CIFAR10), CIFAR10 (for SVHN), KMNIST, and F-MNIST as OOD data across different DNN architectures such as ResNet34, WideResNet, DenseNet, and LeNet5.

==> background.tex <==
\section{Background}
\label{sec:background}
Define OODs- Not seen during training, different from the dataset our classifier is trained on..

==> taxonomy-old.tex <==

\section{OOD Taxonomy and Existing Detection Methods}
\label{sec:taxonomy}
We consider a DNN, trained on the in-distribution samples, to detect OOD samples. Based on the uncertainties associated with the samples, we characterize ODD samples in two categories: epistemic and aleatoric~\citep{uncertainty, ML-uncertainty-survey}. 

\noop{
Beyond the simple characterization of OOD samples as anomalous inputs with respect to the training data, we 
%adopt the top-down inference for a more fine-grained definition of OOD that 
take into account the prediction of the DNN model on the input in determining whether it is OOD or not. This ensures 
%we can take into account 
characterizing both the epistemic and aleatoric uncertainty~\citep{uncertainty}.
%and enables the use of distributions learned individually over the training samples of each class along with the tied distribution learned across classes.
}



\begin{wrapfigure}{r}{0.6\textwidth}
%  \begin{minipage}[c]{0.7\textwidth}
   \begin{center}
    \includegraphics[width=0.6\textwidth]{figures/ood_types_dist_boundary.pdf}
    \caption{The different types of OODs in a 2D space with three different classes. The class distributions are represented as Gaussians with black boundaries and the tyied distribution is a Gaussian with red boundary. }
    \label{fig:OOD_types}
       \end{center}
%  \end{minipage}
 %\begin{minipage}[c]{0.5\textwidth}
%\end{minipage}
%\end{figure}
\end{wrapfigure}

\AR{
\indent \textbf{Taxonomy of OODs.}
%Uncertainty in the prediction of a classifier can be used to detect OODs. We consider aleatory and epistemic as the two sources of this uncertaint. 
% Epistemic uncertainty arises due to the lack of the classifier's knowledge (such as limited training data) whereas aleatory uncertainty is due to the stochasticity (or randomness) involved in its prediction.  
Given a test sample, we analyze the DNN's prediction compared to the in-distribution class boundaries. An OOD sample is associated with aleatoric uncertainty when the DNN may confuse the sample with multiple in-distribution classes (Type 3 OODs in Fig.~\ref{fig:OOD_types}). In case of the epistemic uncertainty, a sample is less likely to belong any of the in-distribution classes (Type 1 OODs in Fig.~\ref{fig:OOD_types}). The uncertainty in the classifier's prediction can thus be quantified with a distance measure from the distribution(s) of the in-distribution samples. \RK{Do we want t osay something about OOD Type 2 here?}

In case of epistemic uncertainty, either a single distribution is estimated for all the in-distribution samples or a class-wise distribution is estimated to capture conditional epistemic uncertainty. Based on the conditional epistemic uncertainty, epistemic uncertainty can be further divided into two types: \textcolor{red}{1) with high variance along the principal components, 2) with relatively low variance across invariant components.}

To this end, we identify an OOD using the following three criteria. 
\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD samples are associated with higher epistemic or aleatoric uncertainty, i.e., is the input away from all in-distribution data or can it be confused between multiple classes? 
    \item Is the epistemic uncertainty of an OOD sample is unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
\end{enumerate}

Figure~\ref{fig:OOD_types} demonstrates different types of OOD which differ along these criteria. Type 1 OOD samples have high epistemic uncertainty and are away from the in-distribution data. Type 2 OOD samples have high epistemic uncertainty with respect to each of the 3 classes even though approximating distribution of all in-distribution data will miss these outliers. Type 3 OOD samples have high aleatoric uncertainty as they are close to the decision boundary between class 0 and class 1. Type 4 and 5 have high epistemic uncertainty with respect to the closest class. While Type 4 OOD samples are far from the distribution along the principal axis, Type 5  OOD samples vary along a relatively invariant axis where even a small deviation indicates an OOD. 

In general, for $k$ number of classes $c_1, c_2, \ldots, c_k$, we denote the distribution of training data for each class as $p(x | c_i)$. The overall training distribution is denoted by $p(x)$. Given a new input $\newinp$ to the trained DNN model $M$, let $\newclass = M(\newinp)$ denote the predicted class. The flowchart in Figure~\ref{fig:OOD_flow} shows the steps to determine whether $\newinp$ is an OOD sample.
}




\noop{
\indent \textbf{Taxonomy of OODs. }
%Uncertainty in the prediction of a classifier can be used to detect OODs. We consider aleatory and epistemic as the two sources of this uncertaint. 
% Epistemic uncertainty arises due to the lack of the classifier's knowledge (such as limited training data) whereas aleatory uncertainty is due to the stochasticity (or randomness) involved in its prediction.  
DNN models predict the class of a new input based on the learned classification boundaries between the distribution of the training samples of different classes. Aleatory uncertainty occurs in the regions where these distributions overlap for multiple classes, and epistemic uncertainty occurs in the regions where the probability of a sample belonging to any of the class distributions is low~\citep{ML-uncertainty-survey}. 
The uncertainty in the classifier's prediction can thus be quantified with a distance measure from the distribution(s) of the training samples. A sample lying close to multiple classes forms the source of aleatory uncertainty and a sample lying far from all the class distributions forms the source of epistemic uncertainty. In the latter case, the distribution of the training samples can be approximated either by a single tied distribution of the entire dataset or class-wise distributions defined by different classes in the dataset. The OODs due to high conditional epistemic uncertainty can be further divided into two types - those with high variance along the principal components and those with relatively low variance across invariant components.
We can thus identify an OOD using the following three criteria. 
\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD input having higher epistemic or aleatoric uncertainty, that is, is the input away from all training data or is it unusually more confusing? 
    \item Is the epistemic uncertainty of the OOD input unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
\end{enumerate}

Figure~\ref{fig:OOD_types} demonstrates different types of OOD which differ along these criteria. Type 1 OODs have high epistemic uncertainty and are away from the training data. Type 2 OODs have high epistemic uncertainty with respect to each of the 3 classes even though approximating distribution of all training data will miss these outliers. Type 3 OODs have high aleatoric uncertainty as they are close to the decision boundary between class 0 and class 1. Type 4 and 5 have high epistemic uncertainty with respect to the closest class. While Type 4 OODs are far from the distribution along the principal axis, Type 5  OODs vary along a relatively invariant axis where even a small deviation indicates an OOD. 

\noop{
In general, 
let there be $k$ classes $c_1, c_2, \ldots, c_k$ and the distribution of training data for each class is $p(x | c_i)$. The overall training distribution is denoted by $p(x)$. Now, given a new input $\newinp$ to the trained DNN model $M$, let $\newclass = M(\newinp)$ denote the predicted class. The flowchart in Figure~\ref{fig:OOD_flow} shows different sources of uncertainty that could make  $\newinp$ an OOD.
}


\begin{figure}[!h]
\centering
\includegraphics[scale=.45]{figures/OOD-flow.png}
\caption{OODs with High Epistemic and Aleatoric Uncertainty} 
\label{fig:OOD_flow}
\end{figure}
}



\noop{
Table~\ref{table:OOD_types} summarizes the taxonomy of OODs based on the distance from the in-distribution and the source of uncertainty. In case of a single tied in-distribution, the only source of uncertainty is the epistemic uncertainty. We classify those samples that lie far from the approximated tied in-distribution as the OODs due to the epistemic uncertainty in the tied in-distribution. Examples of these types of OODs are shown as the black colored OODs in Figure~\ref{fig:OOD_types}. In case of class-wise distribution of the training samples, both epistemic and aleatory can be the source of uncertainty. We classify the samples lying close to multiple class distributions as the OODs due to the aleatory uncertainty in the class-wise in-distribution. Examples of these OODs are shown as the red colored OODs in Figure~\ref{fig:OOD_types}. Those samples that lie far from all the class distributions are classified as the OODs due to the epistemic uncertainty in the class-wise distribution of the in-distribution. 
\begin{table}[!h]
\caption{Taxonomy of OODs}
\label{sample-table}
\begin{center}
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf OOD Type}  &\multicolumn{1}{c}{\bf Source of uncertainty}
\\ \hline \\
Far from tied in-distribution                                   & Epistemic\\
Far from all classes in class-wise in-distribution              & Epistemic\\
Close to multiple class in class-wise in-distribution           & Aleatory\\

\end{tabular}
\end{center}
\label{table:OOD_types}
\end{table}
}


%##########################################################################
%##########################################################################
%##########################################################################


%\subsection{Decomposed Distribution of OODs}

%Further, the OOD due to high epistemic uncertainty can be further divided into two types - those detected by tied distribution across classes and those that are far from all individual classes but not detected by tied distribution due to approximation. The OODs due to high conditional epistemic uncertainty can be further divided into two types - those with high variance along the principal components and those with relatively low variance across invariant components. %These 5 types of OODs are shown in Figure~\ref{fig:OOD_types}. 

%While measuring the distance of a new sample from the learned distribution to estimate $p(\newinp|\newclass)$, we can decompose the input and the training data into a set of orthogonal components and then weigh the component-wise distance from the learned distributions based on the variance of training data along different components. Outliers can have small variance around invariant components or unusually large variance around principle components.
%Decomposing the data along different components with different levels of variation in the training data enables decomposed specification of outliers, and 
%Directly computing outlier metrics such as Mahalanobis distance in the original dimensions of the input does not distinguish between .





%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################


%Three blobs of data-points representing the three types of OODs were used in this example. 

\indent \textbf{Prior Work: Limitations of \textbf{UNIFORM} Detection Methods.} We empirically demonstrate the limitations of existing \RK{not sure if we should say existing or uniform OOD detection techniques} OOD detection methods on a two-dimensional (2D) half-moon dataset with two classes. We assume the samples from the two half-moons to be ID and consider three clusters of OOD samples as shown in Fig.~\ref{fig:toy_ex} (left). \textcolor{red}{We consider a DNN classifier with three fully connected layers having 50, 2, and 2 neuron, respectively.} Figure~\ref{fig:toy_ex} (right) shows the 2D penultimate features of the classifier. The cluster A (black), cluster B (brown), and  cluster C (red) clusters represent the OOD due to epistemic uncertainty in the \textcolor{red}{tied ID}, epistemic uncertainty in the class-conditional ID and aleatoric uncertainty in the class-conditional ID, respectively.

\begin{figure}[!h]
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figures/taxonomy-sec/input_classifier_boundary.pdf}
  %\caption{} 
  %\label{fig:sfig1}
\end{subfigure}%
\quad
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figures/taxonomy-sec/penul_input_with_OOD_types.pdf}
 % \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\caption{We use two half-moons to represent the distribution of the two classes in a 2D dataset. (Left) shows the ID samples and the three clusters of OODs in the input space with the trained classifier's boundary and its softmax scores. (Right) shows the ID samples and the OODs in the 2D penultimate feature space of the classier.} 
\label{fig:toy_ex}
\end{figure}


\begin{figure}[!h]
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of tied in-distribution to detect OODs in cluster B and C.}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/mahala_tied_dist_penul.pdf}}
%  \end{minipage}
  \quad
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the softmax score based technique to detect OODs in cluster A}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/base_classifier_boundary.pdf}}
%  \end{minipage}
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of the class-wise in-distribution to detect OODs in cluster C}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/pca_penul.pdf}}
%  \end{minipage}
  \quad
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the non-conformance among the nearest neighbors to detect OODs in cluster A and B}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/knn_label_conformance_penul.pdf}}
 % \end{minipage}
\caption{Different detection techniques differ in their ability to detect different types of OODs. We call OODs due to epistemic uncertainty in tied ID, class-conditional epistemic uncertainty and aleatoric uncertainty as OODs in cluster A, B and C respectively.}
\label{fig:failure_toy_ex}
\end{figure}



Different approaches differ in their ability to detect different classes of OODs. % described in the previous section. 
First, detection techniques based on density estimation of the tied ID of all the training data do not consider the class of datapoints. Hence, these cannot detect OODs due to the aleatory or epistemic uncertainty in the class-wise distribution.
The estimated tied distribution is overapproximate and it also cannot recognize confusing inputs between different classes.
%over-approximates the in-distribution data  to learn a single distribution and cannot recognize inputs as being confusing between different classes. 
Second, OOD detection techniques based on the softmax prediction probability(SPB) can detect OODs with high aleatoric uncertainty and inter-class confusion. But these are unable to detect the OODs with epistemic uncertainty in the tied ID. This is because of the high softmax scores usually assigned to the samples lying far from the classification boundary by the DNN classifiers. 
Third, OOD detection techniques based on density estimation of the class-wise ID might not be able to detect OODs with high aleatory uncertainty unless we perform counterfactual analysis with classes alternative to the predicted class. 
%OOD detection techniques for class-wise in-distribution 
Finally, the techniques based on the non-conformance amongst the properties of the nearest neighbors from the training samples might not be able to detect OODs due to epistemic uncertainty (in class-wise or tied in-distribution) whose nearest neighbors belong to the same class. 
%This is because training samples from the same class are expected to be conformant in their properties. 

Using the toyset, we empirically demonstrated these limitations of existing OOD detection techniques as summarized in Figure~\ref{fig:failure_toy_ex}. 
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item Mahalanobis distance~\citep{mahalanobis}: 
     A variation in the Mahalanobis distance based method is considered here. Instead of using class-conditional mean and tied covariance, tied mean and tied covariance of all the training data in the penultimate feature space is considered here. This is done to estimate the single tied probability density of all the training data. The  Mahalanobis distance of a new input from this estimated density is then used to distinguish OODs from ID samples. It attains the true negative rate (TNR) of 39.09\% at  the 95\% true positive rate (TPR). It could not detect OODs 
     in clusters B and C, as shown in Figure~\ref{fig:failure_toy_ex}(a).
     \item Softmax prediction probability (SPB)~\citep{baseline}: Figure~\ref{fig:failure_toy_ex}(b) shows that the SPB method cannot  detect the OODs in cluster A. The TNR ( at 95\% TPR) reported by the SPB technique is 60.91\%.  
     \item Class-wise Principal Component Analysis (PCA)~\citep{pca}: We performed PCA of the two classes separately in the penultimate feature space and used the minimum reconstruction error to detect OODs. 
     %The minimum reconstruction error from the principal component of the two classes was used to distinguish OODs from the ID samples. 
     This obtained  TNR of 80.91\% (at 95\% TPR). But it could not detect the OODs in cluster C, as illustrated in Figure~\ref{fig:failure_toy_ex}(c). 
     \item K-Nearest Neighbor (kNN)~\citep{dknn}:  We also used non-conformance (measured as entropy of features in the penultimate layer) in the labels of the nearest neighbors from the ID samples to detect OODs. 
     The TNR (at 95\% TPR) reported by this technique was 15\%. As shown in Figure~\ref{fig:failure_toy_ex}(d), this technique cannot  detect OODs in clusters A and B. 
\end{itemize} 












\noop{
\section{OOD Taxonomy and Existing Detection Methods}

Beyond the simple characterization of OOD samples as anomalous inputs with respect to the training data, we adopt the top-down inference for a more fine-grained definition of OOD that takes into account the prediction of the DNN model on the input in determining whether it is OOD or not. This ensures we can take into account both the epistemic and aleatoric uncertainty~\citep{uncertainty}, and enables the use of distributions learned individually over the training samples of each class along with the tied distribution learned across classes.
\label{sec:taxonomy}
\subsection{Taxonomy of OODs}
%Uncertainty in the prediction of a classifier can be used to detect OODs. We consider aleatory and epistemic as the two sources of this uncertaint. 
% Epistemic uncertainty arises due to the lack of the classifier's knowledge (such as limited training data) whereas aleatory uncertainty is due to the stochasticity (or randomness) involved in its prediction.  
DNN models predict the class of a new input based on the learned classification boundaries between the distribution of training samples of different classes. Aleatory uncertainty occurs in the regions where these distributions overlap for multiple classes, and epistemic uncertainty occurs in the regions where the probability of a sample belonging to any of the class distributions is low~\citep{ML-uncertainty-survey}. 
The uncertainty in the classifier's prediction can thus be quantified with a distance measure from the distribution(s) of the training samples. A sample lying close to multiple classes forms the source of aleatory uncertainty and a sample lying far from all the class distributions forms the source of epistemic uncertainty. In the latter case, the distribution of the training samples can be approximated either by a single tied distribution of the entire dataset or class-wise distributions defined by different classes in the dataset. 

Let there be $k$ classes $c_1, c_2, \ldots, c_k$ and the distribution of training data for each class is $p(x | c_i)$. The overall training distribution is denoted by $p(x)$. Now, given a new input $\newinp$ to the trained DNN model $M$, let $\newclass = M(\newinp)$ denote the predicted class. If $\newinp$ is an OOD, we can identify it using the following three criteria. Figure~\ref{fig:OOD_types} demonstrates different types of OOD which differ along these criteria. 
\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD input having higher epistemic or aleatoric uncertainty, that is, is the input away from all training data or is it unusually more confusing? 
    \item Is the epistemic uncertainty of the OOD input unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
\end{enumerate}


\begin{figure}[!h]
\centering
\includegraphics[scale=.45]{figures/OOD-flow.png}
\caption{OODs with High Epistemic and Aleatoric Uncertainty}
\label{fig:OOD_flow}
\end{figure}




\noop{
Table~\ref{table:OOD_types} summarizes the taxonomy of OODs based on the distance from the ID and the source of uncertainty. In case of a single tied ID, the only source of uncertainty is the epistemic uncertainty. We classify those samples that lie far from the approximated tied ID as the OODs due to the epistemic uncertainty in the tied ID. Examples of these types of OODs are shown as the black colored OODs in Figure~\ref{fig:OOD_types}. In case of class-wise distribution of the training samples, both epistemic and aleatory can be the source of uncertainty. We classify the samples lying close to multiple class distributions as the OODs due to the aleatory uncertainty in the class-wise ID. Examples of these OODs are shown as the red colored OODs in Figure~\ref{fig:OOD_types}. Those samples that lie far from all the class distributions are classified as the OODs due to the epistemic uncertainty in the class-wise distribution of the ID. Examples of these OODs are shown as the brown, magenta and orange colored OODs in Figure~\ref{fig:OOD_types}. 

\begin{table}[!h]
\caption{Taxonomy of OODs}
\label{sample-table}
\begin{center}
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf OOD Type}  &\multicolumn{1}{c}{\bf Source of uncertainty}
\\ \hline \\
Far from tied ID                                   & Epistemic\\
Far from all classes in class-wise ID              & Epistemic\\
Close to multiple class in class-wise ID           & Aleatory\\

\end{tabular}
\end{center}
\label{table:OOD_types}
\end{table}
}

%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################


%\subsection{Decomposed Distribution of OODs}

While measuring the distance of a new sample from the learned distribution to estimate $p(\newinp|\newclass)$, we can decompose the input and the training data into a set of orthogonal components and then weigh the component-wise distance from the learned distributions based on the variance of training data along different components. Outliers can have small variance around invariant components or unusually large variance around principle components.
%Decomposing the data along different components with different levels of variation in the training data enables decomposed specification of outliers, and 
%Directly computing outlier metrics such as Mahalanobis distance in the original dimensions of the input does not distinguish between .





%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################


\subsection{Limitation of Existing OOD Detection Approaches}
Different approaches differ in their ability to detect a different class of OODs described in the previous section. First, OOD detection techniques based on density estimation of the tied ID model all of the training data without considering the class of datapoints. Hence, these cannot detect OODs due to the aleatory or epistemic uncertainty in the class-wise distribution.
The tied distribution over-approximates the ID data to learn a single distribution and cannot recognize inputs as being confusing between different classes. Second, OOD detection techniques based on the softmax scores can detect OODs with high aleatoric uncertainty and inter-class confusion. But these are unable to detect the OODs with epistemic uncertainty in the tied ID. This is because of the high softmax scores usually assigned to the samples lying far from the classification boundary by the DNN classifiers. 
Third, OOD detection techniques based on density estimation of the class-wise ID might not be able to detect OODs with high aleatory uncertainty unless we perform counterfactual analysis with classes alternative to the predicted class. 
%OOD detection techniques for class-wise ID 
Finally, the techniques based on the non-conformance amongst the properties of the nearest neighbors from the training samples might not be able to detect OODs due to epistemic uncertainty (in class-wise or tied ID) whose nearest neighbors belong to the same class~\citep{dknn}.
%This is because training samples from the same class are expected to be conformant in their properties. 
\sj{Ramneet, please add references}.

\textbf{Toy dataset to analyze existing methods.} We empirically demonstrate  these limitations of existing OOD detection methods with the help of a simple 2-dimensional (2D) ID dataset with two classes. Two half-moons represent the distribution of the two classes in this dataset. We trained a classifier with three fully connected layers having 50, 2 and 2 ReLU units, respectively.
%Three blobs of data-points representing the three types of OODs were used in this example. 
Figure~\ref{fig:toy_ex} shows the dataset and the three blobs of OODs in the 2D input and the 2D penultimate feature space of the classifier. The black, brown and red colored blobs of OODs shown in the input space  represent the OODs due to epistemic uncertainty in the tied ID, epistemic uncertainty in the class-wise ID and aleatory uncertainty in the class-wise ID, respectively. The figure also shows the classifier boundary with the softmax scores in the input space.

\begin{figure}[!h]
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/section-3/input_with_OOD_types.pdf}
  \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/section-3/penul_input_with_OOD_types.pdf}
  \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/section-3/classifier_boundary.pdf}
  \caption{}
  %\label{fig:sfig2}
\end{subfigure}
\caption{We use two half-moons to represent the distribution of the two classes in a 2D  dataset. (a) shows the ID samples and the three blobs of OODs in the 2D input space. (b) shows the ID samples and the OODs in the 2D penultimate feature space of the classier and
(c) shows the classifier boundary with softmax scores in the input space. \sj{Please remove whitespaces around pdf or in someway increase font of the text in figures.}}
\label{fig:toy_ex}
\end{figure}

We used Mahalanobis distance from the mean and covariance of the entire dataset as the OOD detection technique based on the density estimation of the tied ID. This mean and covariance was calculated from the penultimate features of the dataset rendered by the classifier. This mahalanobis distance calculated from the tied mean and tied covariance of the dataset was then used to distinguish OODs from ID samples. With the 95\% true positive rate (TPR), the true negative rate (TNR) reported by this technique was 39.09\%. As shown in Figure~\ref{fig:failure_toy_ex}(a), this OOD detection technique based on the density estimation of the tied ID could not detect OODs due to the epistemic and aleatory uncertainty in the class-wise ID.  Figure~\ref{fig:failure_toy_ex}(b) shows that the softmax score used to distinguish OODs from ID samples, again with the 95\% TPR, could not detect the OODs due to the epistemic uncertainty of the tied ID. The TNR reported by this OOD detection technique based on the classifier's softmax scores was 60.91\%.  We performed Principal Component Analysis (PCA) of the two classes separately in the penultimate feature space. The minimum reconstruction error from the principal component of the two classes was used to distinguish OODs from the ID samples.  Although a high TNR of 80.91\% at 95\% TPR was reported by this technique, it could not detect the OODs due to the aleatory uncertainty in the class-wise ID. Figure~\ref{fig:failure_toy_ex}(c) shows the failure of this OOD detection technique based on the density estimation of the individual classes in the dataset. We also used non-conformance in the labels of the nearest neighbors from the ID samples to detect OODs. The entropy of this label distribution in the penultimate feature space was used as a distinguishing measure between the ID samples and OODs. With 95\% TPR, the TNR reported by this technique was 15\%. As shown in Figure~\ref{fig:failure_toy_ex}(d), this technique could not detect OODs due to epistemic uncertainty in both tied and class-wise ID. 

\begin{figure}[t]
  \centering
  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of tied ID to detect OODs due to epistemic and aleatory uncertainty in the class-wise distribution.}
      {\includegraphics[width=1\linewidth]{figures/section-3/mahala_tied_dist_penul.pdf}}
  \end{minipage}\quad
  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the softmax score based technique to detect OODs due to epistemic uncertainty in tied ID}
      {\includegraphics[width=1\linewidth]{figures/section-3/base_classifier_boundary.pdf}}

  \end{minipage}

\bigskip

  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of the class-wise ID to detect OODs due to aleatory uncertainty in class-wise ID}
      {\includegraphics[width=1\linewidth]{figures/section-3/pca_penul.pdf}}

  \end{minipage}\quad
  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the technique based on the non-conformance among the labels of the nearest neighbors in the dataset to detect OODs due to epistemic uncertainty in both tied and class-wise in-distribution}
      {\includegraphics[width=1\linewidth]{figures/section-3/knn_label_conf_penul.pdf}}

  \end{minipage}
\caption{Different OOD detection techniques differ in their ability to detect different types of OODs. \sj{Please increase text fonts without increasing the figure size - increase font size when you are exporting to pdf - also see if you have extra whitespace around figures.}}
\label{fig:failure_toy_ex}
\end{figure}
}


